Bosonic construction of vertex operator para-algebras from symplectic affine Kac-Moody algebras

The representation theory of affine Kac-Moody Lie algebras has grown tremendously since their independent introduction by Robert V. Moody and Victor G. Kac in 1968. Inspired by mathematical structures found by theoretical physicists, and by the desire to understand the ``monstrous moonshine'' of the Monster group, the theory of vertex operator algebras (VOA's) was introduced by Borcherds, Frenkel, Lepowsky and Meurman. An important subject in this young field is the study of modules for VOA's and intertwining operators between modules. Feingold, Frenkel and Ries defined a structure, called a vertex operator para-algebra(VOPA), where a VOA, its modules and their intertwining operators are unified. In this work, for each $l\geq 1$, we begin with the bosonic construction (from a Weyl algebra) of four level $-\shf$ irreducible representations of the symplectic affine Kac-Moody Lie algebra $C_l^{(1)}$. The direct sum of two of these is given the structure of a VOA, and the direct sum of the other two is given the structure of a twisted VOA-module. In order to define intertwining operators so that the whole structure forms a VOPA, it is necessary to separate the four irreducible modules, taking one As the VOA and the others as modules for it. This work includes the bosonic analog of the fermionic construction of a vertex operator superalgebra from the four level 1 irreducible modules of type $D_l^{(1)}$ given by Feingold, Frenkel and Ries. While they only get a VOPA when $l = 4$ using classical triality, the techniques in this work apply to any $l\geq 1$.

==> declare.tex <==
% File:       TeX Inputs declare.tex
% Author:     J E Pittman
% Bitnet:     JEPTeX@TAMVenus
% Internet:   JEPTeX@Venus.TAMU.EDU
% Date:       September 29, 1988
%
% These macros provide a method of locally allocating registers 
% without interference with previously allocated registers.  The 
% method is the same as on pages 346--347 of the \TeX book, however, 
% the declare macros are intended for local use only.  It is a logical 
% error to use a new macro between a declare macro and the end of the 
% appropriate enclosing group. 
%
\def\declarecount {\allocate0\countdef}%
\def\declaredimen {\allocate1\dimendef}%
\def\declareskip  {\allocate2\skipdef}%
\def\declaremuskip{\allocate3\muskipdef}%
\def\declarebox   {\allocate4\chardef}%
\def\declaretoks  {\allocate5\toksdef}%
%
\def\allocate#1#2#3{\relax
   \advance\count1#1 by 1
   \ifnum\count1#1<\count20
   \else
      \errmessage{No room for \string#3!}%
   \fi
   #2#3=\count1#1
   }%
%
\endinput



==> loopy.tex <==
% File:       TeX Inputs loopy.tex
% Author:     J E Pittman
% Bitnet:     JEPTeX@TAMVenus
% Internet:   JEPTeX@Venus.TAMU.EDU
% Date:       September 29, 1988
%
% These macros supply structured, nested loop constructs as follows:
%  
%     \forcount \csname=number to number by number do
%        valid_TeX_input
%        \endfor \csname 
%
%     \while \csname \if_of_any_type do
%        valid_TeX_input
%        \endwhile \csname 
%
%     \whilenot \csname \if_of_any_type do
%        valid_TeX_input
%        \endwhile \csname         
%
% The \csname for the for loop must refer to a count register, for the 
% while loops it must uniquely identify the while loop.
%
\def\forcount #1{\relax
   \def
         \for #1=##1to ##2by ##3do
            ##4%
            \endfor #1%
      {\relax
      #1=##1\relax
      \ifnum ##3>0
         \whilenot #1\ifnum ##2<#1do
            ##4%
            \advance #1 by ##3\relax
            \endwhilenot #1%
      \else
         \while #1\ifnum ##2<#1do
            ##4%
            \advance #1 by ##3\relax
            \endwhile #1%
      \fi
      }%
   \for #1%   
   }%
%
\let\endwhilenot=\fi
%
\def\whilenot #1{\relax
   \def
         \whilenotloop#1 ##1do
            ##2%
            \endwhilenot #1%
      {\relax
         \expandafter\def\csname whilenotbody\string#1\endcsname{##2}%
         \expandafter\def\csname whilenotloop\string#1\endcsname
            {\relax
               ##1%
                  \let\next=\relax
               \else
                  \csname whilenotbody\string#1\endcsname
                  \expandafter\let\expandafter\next
                        \csname whilenotloop\string#1\endcsname
               \fi
               \next
               }%
         \csname whilenotloop\string#1\endcsname
         }%
   \whilenotloop#1
   }%
%
\let\endwhile=\fi
%
\def\while #1{\relax
   \def
         \whileloop#1 ##1do
            ##2%
            \endwhile #1%
      {\relax
         \expandafter\def\csname whilebody\string#1\endcsname{##2}%
         \expandafter\def\csname whileloop\string#1\endcsname
            {\relax
               ##1%
                  \csname whilebody\string#1\endcsname
                  \expandafter\let\expandafter\next
                        \csname whileloop\string#1\endcsname
               \else
                  \let\next=\relax
               \fi
               \next
               }%
         \csname whileloop\string#1\endcsname
         }%
   \whileloop#1
   }%
%
\endinput


